FusionPortable: A Multi-Sensor Campus-Scene Dataset for Evaluation of Localization and Mapping Accuracy on Diverse Platforms

Combining multiple sensors enables a robot to maximize its perceptual awareness of environments and enhance its robustness to external disturbance, crucial to robotic navigation. This paper proposes the FusionPortable benchmark, a complete multi-sensor dataset with a diverse set of sequences for mobile robots. This paper presents three contributions. We first advance a portable and versatile multi-sensor suite that offers rich sensory measurements: 10Hz LiDAR point clouds, 20Hz stereo frame images, high-rate and asynchronous events from stereo event cameras, 200Hz inertial readings from an IMU, and 10Hz GPS signal. Sensors are already temporally synchronized in hardware. This device is lightweight, self-contained, and has plug-and-play support for mobile robots. Second, we construct a dataset by collecting 17 sequences that cover a variety of environments on the campus by exploiting multiple robot platforms for data collection. Some sequences are challenging to existing SLAM algorithms. Third, we provide ground truth for the decouple localization and mapping performance evaluation. We additionally evaluate state-of-the-art SLAM approaches and identify their limitations. The dataset, consisting of raw sensor easurements, ground truth, calibration data, and evaluated algorithms, will be released: https://ram-lab.com/file/site/multi-sensor-dataset.

==> discussion.tex <==
\section{Dicussion}
\label{sec:discussion}

\bt{jjiao: This section will discuss discoveries from the process of making this dataset and evaluation, like lessons, the raised demand of new evaluation metrics, new research problems or old problems that are not addressed well, etc. }

\subsection{Known Issues}
gt poses are seldom jerky

==> fig_dataformat.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \dirtree{%
  .1 dataset/.
  .2 platform/.
  .3 date\_env/.
  .4 calib/sensor\_name.yaml.
  .4 groundtruth\_traj.txt.
  .4 env.bag, env\_ref.bag.
  .4 data/, data\_ref\_kitti/.
  .5 sensor\_name/.
  .6 data\_type.
  .7 data/frame\_number.(pcd/png).
  .7 timestamps.txt.
  % .6 imu/.
  % .7 data.csv.
  .2 groundtruth\_map/.
  .3 date\_env/.
  .4 scan/scan\_number.pcd.
  .4 merged\_scan.pcd.
  .4 transformation\_scan.yaml.
  } 
  \caption[xx]{Structure of the dataset. 
  Sequences are named as date and environmental description: \texttt{date\_env}.
  Sensor data are stored in files. 
  Here, \texttt{sensor\_name} refers to sensors as \texttt{ouster00}, \texttt{frame\_cam00}, \texttt{frame\_cam01}, \texttt{event\_cam00}, and \texttt{event\_cam01}, and \texttt{data\_type} refers to \texttt{point}, \texttt{image}, \texttt{event}, and \texttt{imu}. Calibration parameters, ground-truth poses, and maps are also contained.}
  \label{fig:dataset_format}
\end{figure}
